ACAP: Asynchronous Coding Agents for Efficient Robot Control

Coding agents can construct and revise robot behavior during execution, but using one agent for the whole robot can delay otherwise independent work. We introduce Asynchronous Coding Agents as Policy (ACAP), an asynchronous framework that organizes one robot as a team of persistent agents. Each member reasons and acts for a configurable control group, such as an arm with its gripper or the torso and chassis, enabling asynchronous reasoning and execution. However, different robot components often have physical dependencies that require coordination. To address this challenge, ACAP introduces a hyper-agent that assigns tasks, coordinates dependencies, and dynamically allocates control between the lead and member agents. This allows independent work to progress concurrently while supporting tightly coupled manipulation when necessary. Across 72 real-world rollouts covering 25 task/platform settings, ACAP reduces task-balanced time cost by 28.2% compared with a single-agent Direct Policy, with improvements across Fully Parallel, Parallel-Sequential, and Collaborative tasks. Across all eight Collaborative settings, ACAP also achieves lower mean time cost than Fixed Delegation, where only member agents can control their assigned groups. An additional 90-rollout study shows lower mean 30-minute-capped time cost than Direct on all six tasks. We further demonstrate mobile manipulation using the same member interface for chassis and torso control. We present the framework and a real-world rollout dataset containing observations, generated programs, actions, and feedback to support research on how coding agents reason and act in the physical world.

==> sections/tables/repeated_instructions.tex <==
Wipe and arrange towels (R1) & Clean up the dirty water with the blue towel. Put the clean white towel rolls into the tray side by side. \\
Sort cubes and batteries (P-B) & Put the cubes into the plate, batteries into the cup. \\
Insert four flowers (P-A) & Insert the flowers into the vase. \\
Assemble a sandwich (P-D) & Insert one piece of lettuce between the two pieces of bread. \\
Fold a towel (P-B) & Fold the towel into a quarter square, from bottom to top, then from left to right. \\
Lift a milk carton (P-A) & Hold the milk brick in the air with both hands, showing a clear margin above the table. \\


==> sections/tables/task_instructions.tex <==
\multicolumn{2}{@{}l}{\textbf{Fully Parallel}} \\*
\midrule
T01 & Put the batteries into their nearest plates. \\
T02 & Put the batteries into their nearest box. \\
T03 & Clean up the dirty water with the blue towel. Put the clean white towel rolls into the tray. \\
T04 & Put the two bottles of water into the tray, upright in the center, then put the rolled towels onto the tray, one on each side. \\
T05 & Put the towel rolls into the tray, side by side. \\
T06 & Put the cubes into the plate, batteries into the cup. \\
\addlinespace
\multicolumn{2}{@{}l}{\textbf{Parallel-Sequential}} \\*
\midrule
T07 & Put the pens into the pen holder. \\
T08 & Insert the plastic flowers into the vase. \\
T09 & Put the items in respective grids. \\
T10 & Insert the plastic flowers into the vase. \\
T11 & Put the pens into the pen holder. \\
T12 & Put the clothes into the basket. \\
T13 & Put the sponge cubes into the tank. \\
T14 & Stack the paper cups to the one marked with X. \\
T15 & Put the toy blocks on the table into the basket. \\
T16 & Stack the towel rolls into a pyramid on the tray, three at the bottom, two in the middle, and one on top. \\
T17 & Insert the plastic flowers into the vase. \\
\addlinespace
\multicolumn{2}{@{}l}{\textbf{Collaborative}} \\*
\midrule
T18 & Fold the towel into a quarter square, from bottom to top, then from left to right. \\
T19 & Lift the basket in the air, and hold still. / Lift the basket in the air, with a clear margin above the table, and hold still. \\
T20 & Fold the T-shirt into a square, from bottom to top. \\
T21 & Twist open the bottle. \\
T22 & Lift the fruit basket in the air, with a clear margin above the table, and hold still. \\
T23 & Hold the milk brick in the air with both hands, showing a clear margin above the table. \\
T24 & Put the pot on the book. \\
T25 & Put the fruit basket onto the black sponge. \\

